Sequencing Matters: A Generate-Retrieve-Generate Model for Building Conversational Agents

This paper contains what the Georgetown InfoSense group has done in regard to solving the challenges presented by TREC iKAT 2023. Our submitted runs outperform the median runs by a significant margin, exhibiting superior performance in nDCG across various cut numbers and in overall success rate. Our approach uses a Generate-Retrieve-Generate method, which we've found to greatly outpace Retrieve-Then-Generate approaches for the purposes of iKAT. Our solution involves the use of Large Language Models (LLMs) for initial answers, answer grounding by BM25, passage quality filtering by logistic regression, and answer generation by LLMs again. We leverage several purpose-built Language Models, including BERT, Chat-based, and text-to-transfer-based models, for text understanding, classification, generation, and summarization. The official results of the TREC evaluation contradict our initial self-evaluation, which may suggest that a decrease in the reliance on our retrieval and classification methods is better. Nonetheless, our findings suggest that the sequence of involving these different components matters, where we see an essentiality of using LLMs before using search engines.

==> intro_flowchart.tex <==
\begin{tikzpicture}[node distance=1.3cm]
\node (userutterance) [io] {\begin{varwidth}{6em}User Utterance\end{varwidth}};
\node (ptkbs) [io,right of=userutterance,xshift=2cm] {\begin{varwidth}{6em}PTKBs\end{varwidth}};
\node (sentance_bert) [process, below of=userutterance] {\begin{varwidth}{8em}Sentence-BERT to Rank PTKBs\end{varwidth}};
\node (query_generator) [process, right of=sentance_bert, xshift=2cm] {\begin{varwidth}{8em}Prompt Generator\end{varwidth}};
\node (llama) [process, left of=query_generator,xshift=-2cm,yshift=-1.5cm] {\begin{varwidth}{8em}LLama2 Response\end{varwidth}};
\node (bm25) [process, below of=llama] {\begin{varwidth}{8em}BM25 on Clueweb-22B\end{varwidth}};
\node (tfidf) [process, below of=bm25] {\begin{varwidth}{8em}Logistic Regression Passage Classifier\end{varwidth}};
\node (relevance) [process, right of=tfidf,xshift=2cm,yshift=2cm] {\begin{varwidth}{8em}Rank Passage Sentence Relevance with Sentence-BERT; Prompt Generator\end{varwidth}};
\node (fastchat) [process, below of=relevance, yshift=-1cm] {\begin{varwidth}{8em}Summarize Passages with FastChat-T5 \& Combine Top n Summaries\end{varwidth}};

\node (twoshot) [decision, right of=relevance,xshift=1.5cm,yshift=1cm] 
{\begin{varwidth}{8em}Yes\end{varwidth}};

\node (is_twoshot) [decision, below of=twoshot,yshift=-.5cm] 
{\begin{varwidth}{5em}Is Two Shot?\end{varwidth}};

\node (oneshot) [decision, below of=is_twoshot] 
{\begin{varwidth}{8em}No\end{varwidth}};

\node (final) [process, below of=oneshot] 
{\begin{varwidth}{8em}Fluent Response Cut-Off\end{varwidth}};
\node (end) [startstop, left of=final,xshift=-1cm,yshift=-.25cm] 
{\begin{varwidth}{15em}End\end{varwidth}};

\draw [arrow] (userutterance) -- (sentance_bert);
\draw [arrow] (ptkbs) -- (sentance_bert);

\draw [arrow] (sentance_bert) -- (query_generator);
\draw [arrow] (query_generator) -- (llama);
\draw [arrow] (llama) -- (bm25);
\draw [arrow] (bm25) -- (tfidf);
\draw [arrow] (tfidf) -- (relevance);
\draw [arrow] (relevance) -- (fastchat); 

\draw [arrow] (fastchat) -- (is_twoshot); 
\draw [arrow] (is_twoshot) -- (twoshot); 
\draw [arrow] (twoshot) -- (llama); 
\draw [arrow] (is_twoshot) -- (oneshot); 
\draw [arrow] (oneshot) -- (final); 
\draw [arrow] (final) -- (end); 
\end{tikzpicture}

==> related.tex <==
\section{Related Work}


% \subsection{Large Language Model Grounding}

After the introduction of Large Language Models such as ChatGPT, many began using them for information retrieval. This came with drawbacks, due to the issues Large Language Models face from hallucinations \cite{zhang2023sirens} and bias \cite{ferrara2023chatgpt}. To augment the text generation capabilities of Large Language Models, many rely on  information retrieval methods to back up outputs with accurate human-generated content.

LLM Grounding methods can be grouped into three categories: Fact-Checking, Generate-From-Information, and Generate-Then-Retrieve. Some approaches work by fact-checking and citing the claims made by the LLM, and rewriting any claim identified as false and/or unciteable \cite{gao2023rarr}. In these approaches, a majority of the text content was LLM generated, which still allows for the conversational and deeper language-understanding benefits of Language Models. However, this still leaves room for model bias, and the process of fact-checking and citing is not 100\% effective. Thus, some approaches \cite{ma2023pretraining} involve relying on human-generated content for the entire response, using Large Language Models solely for their abilities to expand and 'answer' queries, then using that response to retrieve passages that can be summarized or extracted into the final response. We initially considered using a similar approach, although ran into issues with the LLM not solely drawing from given information and instead drawing mostly from its training data. This method does not guarantee full accuracy, and still has the same problems, although to a lesser extent, as just pure generation techniques. Additionally, hybrid methods \cite{huo2023retrieving} use a prompting technique, where they find supporting passages (either from using a LLM response or just the user utterance), then ask the LLM to answer the question from the passage. 

Our approach uses a modified version of the expansion approach - we use the LLM to generate a response to the user utterance with minimal prompting (only providing the relevant PTKBs and utterance combined in a linguistically fluent manner). We encourage the LLM to generate a lengthy response, in order to get more information that can be used to find grounding materials. Even if the LLM states something incorrect, there is a high likelihood that its response will correspond significantly with what the user asked it. Once we've retrieved relevant passages, we then use a text-to-text transfer Large Language Model specifically designed for summarization to summarize each passage, after optimizing the sentences of each passage to prioritize the information actually relevant to the user utterance. Our method maintains the citability of fact-checking-based methods and the conversational fluency enabled by LLMs. Unlike the generate-then-retrieve methods, our approach still involved using an LLM in creating our final response, which allowed for more intelligent and fluent responses. 


